Network Unreliability in Almost-Linear Time

The network unreliability problem asks for the probability that a given undirected graph gets disconnected when every edge independently fails with a given probability $p$. Valiant (1979) showed that this problem is \#P-hard; therefore, the best we can hope for are approximation algorithms. In a classic result, Karger (1995) obtained the first FPTAS for this problem by leveraging the fact that when a graph disconnects, it almost always does so at a near-minimum cut, and there are only a small (polynomial) number of near-minimum cuts. Since then, a series of results have obtained progressively faster algorithms to the current bound of $m^{1+o(1)} + \tilde{O}(n^{3/2})$ (Cen, He, Li, and Panigrahi, 2024). In this paper, we obtain an $m^{1+o(1)}$-time algorithm for the network unreliability problem. This is essentially optimal, since we need $O(m)$ time to read the input graph. Our main new ingredient is relating network unreliability to an {\em ideal} tree packing of spanning trees (Thorup, 2001).

==> proofs.tex <==
\section{Omitted Proof from \Cref{sec:prelim}}
\label{sec:proof2}

\subsection{Proof of \Cref{lem:contract-strong-oneshot}}
    Let the $k$-strong components be $S_1, S_2, \ldots, S_r$, and $H=G/\{S_1,S_2, \ldots, S_r\}$. Let $D[G]$ be the event that $G$ disconnects when each edge fails independently with probability $p$. Use coupling to force the same edge to witness the same outcome in all events. Here the same edge is naturally defined for induced subgraphs and contracted subgraphs.
    When each $G[S_i]$ is connected, and $H$ is also connected, we can concatenate an arbitrary spanning tree of each of them to connect the whole graph $G$. That is,
    \[ (\lnot D[H]) \land \bigwedge_i (\lnot D[G[S_i]]) \implies \lnot D[G] \]
    Equivalently,\[D[G] \implies D[H]\lor \bigvee_i D[G[S_i]].\]
    Notice that the events in RHS are independent because their involved edge sets are disjoint. Taking probability gives
    \[u_G(p) \le u_H(p) + \sum_i u_{G[S_i]}(p).\]
    We also have $D[H]$ implies $D[G]$, so $u_G(p) \ge u_H(p)$. It remains to prove that $\sum_i u_{G[S_i]}(p) \le \eps \cdot u_G(p)$.

    Let $n_i = n_{G[S_i]}, \lambda_i = \lambda_{G[S_i]}$. We have $$\frac{\sum_i u_{G[S_i]}(p)}{u_G(p)} \le \frac{\sum_i n_i^2 p^{\lambda_i}}{p^\lambda} \le  p^{3\lambda-\lambda} \sum_i n_i^2 \le n^2 p^{2\lambda} \le \eps.$$


\section{Omitted Proofs from \Cref{sec:packing}}
\label{sec:proof3}


\subsection{Proof of \Cref{lem:ugp-ktau}}

Form a graph $H$ by contracting all edges $e$ with $\ell^*(e) < \frac{1}{\tau}$. By definition of $k_\tau$, we have $|V(H)|=k_\tau$. Since we set $\ell^*(e)=1/\pi^*$ for at least one edge in the global min-ratio cut, the graph $H$ is not a singleton.

Next, we claim that if we run the recursive min-ratio cut process in $H$, the ideal loads of edges in $H$ are the same as their original ideal loads in $G$.
To see the claim, we need a property that the ideal loads are monotonically non-increasing down the recursion tree (Lemma 14 of \cite{Thorup01}).
Then, contracting edges $e$ with $\ell^*(e)<\frac1\tau$ does not affect recursive instances that set load $\frac{|P|-1}{d(P)}\ge\frac1\tau$. Since there is a fractional tree on $H$ whose edge loads equal $\ell^*$, we have $\ell^*(E(H))=|V(H)|-1=k_\tau-1$.

Let $\bar d$ be the average degree in $H$. We bound
    \[\bar{d} = \frac{1}{k_\tau}\sum_{v\in V(H)} d(v) = \frac{2|E(H)|}{k_\tau} \le \frac{2}{k_\tau} \cdot \ell^*(E(H)) \cdot \tau = 2\tau \cdot \frac{k_\tau-1}{k_\tau}\le 2\tau.\]
Since the degree cut of each vertex $v\in V(H)$ corresponds to a separate cut in $G$, we have
    \[\zgp \ge \sum_{v\in V(H)} p^{d(v)} \ge k_\tau p^{\bar{d}} \ge k_\tau p^{2\tau},\]
where the middle inequality follows by convexity of the function $f(x)=p^x$.

\subsection{Proof of \Cref{cor:greedy-packing}}

We use the following lemma from \cite{Thorup01}:
\begin{lemma}[Proposition 16 of \cite{Thorup01}]\label{lem:greedy-packing}
In an unweighted graph with min-cut value $\lambda$, suppose that $\mathcal{T}$ is a (multi-)set of spanning trees generated by greedy tree packing after $\ge 6\lambda \ln m/\delta^2$ iterations, where parameter $\delta < 2$. Let $\ell^{\mathcal T}$ be the edge loads for the uniform distribution over $\mathcal T$. Then, for all edges $e$,
    $$|\ell^{\mathcal{T}}(e) - \ell^*(e)| \le \delta/\lambda.$$
\end{lemma}

Now, we proceed to prove \Cref{cor:greedy-packing}. 
Compute a tree packing of $N=12\lambda\ln m/\delta^2$ trees, which is twice as many as needed by \Cref{lem:greedy-packing}, and let $\mathcal T$ be the latter $N/2$ of the spanning trees computed. On each iteration $i>6\lambda\ln m/\delta^2$ of greedy tree packing, we have $|\ell^{\mathcal T_i}(e)-\ell^*(e)|\le\delta/\lambda$ for all $e\in E$, where $\mathcal T_i$ is the uniform distribution over the current tree packing of $i-1$ trees. For the next tree $T$ to be packed, define $\ell_T=\ell^{\mathcal T}$, which satisfies property~(2). For property~(1), for each $e\in E$ we have
\[ \ell^{\mathcal T}(e)=\frac{N\cdot\ell^{\mathcal T_N}(e)-N/2\cdot\ell^{\mathcal T_{N/2}}(e)}{N/2}=2\ell^{\mathcal T_N}(e)-\ell^{\mathcal T_{N/2}}(e) ,\]
which together with $|\ell^{\mathcal T_N}(e)-\ell^*(e)|\le\delta/\lambda$ and $|\ell^{\mathcal T_{N/2}}(e)-\ell^*(e)|\le\delta/\lambda$ concludes property~(1).

For the running time, we dynamically maintain the minimum spanning tree over the iterations using, e.g.\ the algorithm of~\cite{holm01}. Each iteration takes $\tilde O(1)$ time to compute the new minimum spanning tree, and then $\tilde O(n)$ time to update the weights on each edge of the spanning tree. The total running time over the $\tilde O(\lambda/\delta^2)$ iterations is $\tilde O(\lambda/\delta^2)\cdot\tilde O(n)=\tilde O(m/\delta^2)$ since $m\ge n\lambda/2$.



\subsection{Proof of \Cref{lem:load-range}}

%Let $P^*$ be the partition with the min-cut ratio $\pi^*$. The degree cut values of the $|P^*|$ components sum to $2d(P)$ and therefore have average value $\frac{2d(P)}{|P|}$, which is at least $\lambda$. We obtain $2\pi^*\ge\frac{2d(P)}{|P|}\ge\lambda$. Since edge loads are monotonically decreasing in the recursive ideal load algorithm, each edge has ideal load at most $1/\pi^*\le2/\lambda$.
By \Cref{fact:pi-range}, $1/\pi^* < 2/\lambda$. Since edge loads are monotonically decreasing in the recursive ideal load algorithm, each edge has ideal load less than $2/\lambda$.

For a given uncontracted edge $e$ of strength less than $3\lambda$, consider an instance $G[S]$ in the recursive load algorithm whose min-ratio cut sets value $\ell^*(e)$. Since $G[S]$ contains edge $e$ of strength $< 3\lambda$,  the min-cut value of $G[S]$ is $< 3\lambda$. By definition of $\ell^*(e)$, the minimum cut ratio of $G[S]$ is $\frac{1}{\ell^*(e)}$. Any (2-way) cut is a partition whose cut ratio equals the cut value. So, the connectivity of $G[S]$ is no less than the value of the min-ratio cut. Denoting by $\lambda_{G[S]}$ the minimum cut of $G[S]$, we conclude that $\frac{1}{\ell^*(e)} \le \lambda_{G[S]} < 3\lambda$, which implies $\ell^*(e) > \frac{1}{3\lambda}$.



\subsection{Proof of \Cref{lem:tilde-ki-range}}
By property~(1) of \Cref{cor:greedy-packing}, we have $|\ell^{\mathcal{T}}(e) - \ell^*(e)| \le 3\eps$ for all edges $e$.
By property~(2) of \Cref{cor:greedy-packing}, each tree $T\in\mathcal T$ is the MST of some weight function $\ell_T$ satisfying $|\ell_T(e)-\ell^*(e)|\le\eps$ for all $e\in E$. Combining the two properties, we obtain $|\ell_T(e)-\ell^{\mathcal T}(e)|\le4\eps$ for all $e\in E$. We can set $\eps=\Theta(\delta/\lambda)$ small enough that $\ell^{\mathcal T}(e)\approx_\delta\ell^*(e)$ and $\ell_T(e)\approx_\delta\ell^{\mathcal T}(e)$ for all $e\in E$. 

For the first statement, observe that
\[ e\in\widetilde E_{>i+1}\implies\ell^{\mathcal T}(e)<\frac1{\pi_{i+1}}\implies\ell^*(e)<\frac1{\pi_i}\implies e\in E_{>i} ,\]
so $\widetilde E_{>i+1}\subseteq E_{>i}$, and it follows that $k_{\pi_i}\le\tilde k_{\pi_{i+1}}$. The other inequality $\tilde k_{\pi_{i+1}}\le k_{\pi_{i+2}}$ follows by an identical argument.

For the second statement, we have
\begin{align*}
e\in\widetilde E_{>i+2}&\implies \ell^{\mathcal T}(e) < \frac{1}{\pi_{i+2}} \implies \ell_T(e) < \frac{1}{\pi_{i+1}} , \quad\text{and}
%\\ e\in E_i&\implies \ell^*(e) \ge \frac{1}{\pi_i} \implies \ell_T(e) \ge \frac{1}{\pi_{i+1}} ,
\\ e\in\widetilde E_{i} &\implies \ell^{\mathcal T}(e) \ge \frac{1}{\pi_i} \implies \ell_T(e) \ge \frac{1}{\pi_{i+1}}.
\end{align*}
Imagine running Kruskal's MST algorithm on weight function $\ell_T$. All edges in $\widetilde E_{>i+2}$ are prioritized over all edges in $\widetilde E_i$, so by the time an edge in $\widetilde E_i$ is visited by Kruskal's algorithm, the current spanning forest has at most $\tilde k_{\pi_{i+2}}$ connected components. It follows that there are at most $k_{\pi_{i+2}}-1$ edges in $\widetilde E_i$ added to $T$.



\subsection{Proof of \Cref{lem:ignore-cuts-log-n}}
Equivalently, we need to prove that $z_G(p)-z'_G(p)\le O(1/n)z_G(p)$, where $z_G(p)-z'_G(p)=\sum_{C\notin\mathcal C}p^{|C|}$. Define $\mathcal C'$ as the collection of cuts $C$ with $\ell^*(C)\le\log n$. Since $\ell^{\mathcal T}(e)\approx_\delta\ell^*(e)$ for all $e\in E$, any cut with $\ell^*(C)\le\log n$ also satisfies $\ell^{\mathcal T}(C)\le2\log n$, so $\mathcal C'\subseteq\mathcal C$. So it suffices to show that $\sum_{C\notin\mathcal C'}p^{|C|}\le O(1/n)z_G(p)$.
We have two cases depending on whether $p^\lambda > n^{-2}/\log n$.

Assume first that $p^\lambda > n^{-2}/\log n$. Consider a fixed cut $C$, and let $C_i$ be the cut edges on level $i$.
Since the min-ratio cut algorithm sets $\ell^*(e)=\frac1{\pi_i}$ for all edges $e\in C_i$, we have $|C|=\sum_i\ell^*(C_i)\pi_i$. From the assumption, we have $p^{\pi_i}\le(\max\{k_{\pi_i},\sqrt n\})^{-(1+\delta)}$ for all $i$. We bound
\begin{align}
    \sum_{C\notin\mathcal C'}p^{|C|} = \sum_{C:\ell^*(C) > \log n} p^{|C|} &=  \sum_{C:\ell^*(C) > \log n} \prod_i p^{\ell^*(C_i) \pi_i}\nonumber
    \\&\le\sum_{C:\ell^*(C) > \log n}  \prod_i (\max\{k_{\pi_i},\sqrt n\})^{-(1+\delta)\ell^*(C_i)}\label{eq:zL}
.
\end{align}
We now bound the number of cuts $C$ with $\ell^*(C)=\alpha$ for a given $\alpha$.
For each cut $C$, if we take a sample $T$ from the ideal tree packing, we obtain $\mathbb E[|C\cap T|]=\ell^*(C_i)$. By Markov's inequality, with probability at most $(1+\delta/2)^{-1}$ the sampled tree $T$ satisfies $|C_i\cap T|>(1+\delta/2)\ell^*(C_i)$. So with probability $\Omega(\delta)$, we have $|C_i\cap T|\le(1+\delta/2)\ell^*(C_i)$. We can sample a tree from the ideal tree packing such that the $k_{\pi_i}-1$ edges of the tree on each level $i$ are independent. So with probability $\Omega(\delta)^{O(1/\delta)}$, we have $|C_i\cap T|\le(1+\delta/2)\ell^*(C_i)$ for all $i$. 
This probability is for a random tree in packing. So, if the tree packing has size at least $O(1/\delta)^{O(1/\delta)}$, then there exists a tree $T$ to make it happen. It follows that for any collection of integers $\{\alpha_i\}_i$ there are at most $O(1/\delta)^{O(1/\delta)}\cdot\prod_ik_{\pi_i}^{(1+\delta/2)\alpha_i}$ many cuts $C$ with $|C_i\cap T|=\alpha_i$ for all $i$. Continuing from (\ref{eq:zL}), we union bound over all $\{\alpha_i\}_i$ summing to $\alpha\ge\log n$ to get
\begin{align*}
\sum_{C\notin\mathcal C'}p^{|C|}&\le\sum_{\alpha\ge\log n}\sum_{\sum_i\alpha_i=\alpha} O(1/\delta)^{O(1/\delta)}\cdot\prod_ik_{\pi_i}^{(1+\delta/2)\alpha_i}\cdot \prod_i (\max\{k_{\pi_i},\sqrt n\})^{-(1+\delta)\alpha_i}
\\&\le\sum_{\alpha\ge\log n}\sum_{\sum_i\alpha_i=\alpha}O(1/\delta)^{O(1/\delta)}\cdot\prod_i(\max\{k_{\pi_i},\sqrt n\})^{-\delta\alpha_i}
\\&\le\sum_{\alpha\ge\log n}\sum_{\sum_i\alpha_i=\alpha}O(1/\delta)^{O(1/\delta)}\cdot\prod_i(\sqrt n)^{-\delta\alpha_i}
\\&\le\sum_{\alpha\ge\log n}\sum_{\sum_i\alpha_i=\alpha}O(1/\delta)^{O(1/\delta)}\cdot n^{-\delta\alpha/2}.
\end{align*}
For a fixed integer $\alpha$, there are at most $\binom{\alpha}{O(1/\delta)}$ ways to write it as $\alpha=\sum_i\alpha_i$, so the expression above is at most
\[ \sum_{\alpha\ge\log n}\alpha^{O(1/\delta)}\cdot O(1/\delta)^{O(1/\delta)}\cdot n^{-\delta\alpha/2}\le(\log  n)^{O(1/\delta)}\cdot O(1/\delta)^{O(1/\delta)}\cdot n^{-\delta(\log n)/2}\le n^{o(1)-\frac{\log n}{2\log \log n}}\le O(1/n)\cdot p^\lambda, \]
concluding the case $p^\lambda > n^{-2}/\log n$.

Next, assume that $p^\lambda \le n^{-2}/\log n$. Observe that any cut $C$ with $\ell^*(C)\ge\log n$ satisfies $|C| = \sum_i |C_i| \ge \sum_i \ell(C_i)\pi_i\ge\sum_i\ell(C_i)\pi^*\ge\log n \cdot \lambda/2$, i.e., it is a $(\frac12\log n)$-approximate minimum cut.
We use $z\ge p^\lambda$ and the standard cut-counting argument to get
    \begin{align*}
    \frac1z\sum_{C\notin\mathcal C'}p^{|C|} 
    &\le p^{-\lambda}\sum_{j \ge\frac12\log n}n^{2(j+1)}p^{j\lambda}
    = n^4\sum_{j \ge\frac12\log n}n^{2(j-1)}p^{(j-1)\lambda}\\
    &= n^4\sum_{j \ge\frac12\log n}(n^2p^\lambda)^{j-1}
    \le n^4\cdot O\left(\frac{1}{\log n}\right)^{\log n/2},
    \end{align*}
    which is at most $O(1/n)$, concluding the proof.

\subsection{Proof of \Cref{lem:criteria-inverse}}
\alert{
First, we consider the case when $\tilde{k}_{\pi_i} = 1$. The assumption becomes $p^{2\pi_i} > n^{-1-30\delta}$.
Since $\pi_i \ge \pi_0=\lambda/2$, this implies
$p^{\lambda}\ge p^{2\pi_i} > n^{-1-30\delta}$, which further implies $\ugp \ge n^{-1-O(1/\log \log n)}$.

Next, we consider the case when $\tilde{k}_{\pi_i} > 1$. 
Recall that $\tilde{k}_{\pi_i}$ is the number of nodes after contracting edges with $\ell^{\mathcal{T}}(e) < \frac{1}{\pi_i}$. So, in this case, there exists an edge $e$ with $\ell^{\mathcal{T}}(e) \ge \frac{1}{\pi_i}$. Since $\ell^{\mathcal{T}}(e)\approx_\delta \ell^*(e)$, we have $\pi^* \le \frac{1}{\ell^*(e)} \le (1+\delta)\pi_i = \pi_{i+1}$. %\textcolor{blue}{Jason: Isn't $\pi^*$ the maximum $\ell^*(e)$ over all $e$ ? How is this possible? May have to do with my comment in the statement of \Cref{lem:ugp-ktau}.} 
So, we can apply \Cref{lem:ugp-ktau} to get $\zgp \ge k_{\pi_{i+1}} p^{2\pi_{i+1}}$.
}
    From the assumption, we have
    \[1 <  n^{1+30\delta} \tilde k_{\pi_i} p^{2 \pi_i} \le n^{1+30\delta} k_{\pi_{i+1}} p^{2 \pi_i}=n^{1+30\delta}k_{\pi_{i+1}}p^{2\pi_{i+1}/(1+\delta)},\]
    where the inequality uses \Cref{lem:tilde-ki-range}.
    Combined with \Cref{lem:ugp-ktau}, we have
    \[(\zgp)^{1/(1+\delta)} \ge (k_{\pi_{i+1}})^{1/(1+\delta)}p^{2\pi_{i+1}/(1+\delta)}=k_{\pi_{i+1}}(k_{\pi_{i+1}})^{-O(\delta)}p^{2\pi_{i+1}/(1+\delta)}\ge n^{-(1+30\delta)}k^{-O(\delta)} \ge n^{-1-O(\delta)}.\]
    Therefore, $\zgp > n^{-1-O(\delta)}$ as claimed. Combined with \Cref{lem:z-approx-u} that $\ugp \ge (1-\frac{1}{\log n})\zgp$ when $p\le \theta$, we have $\ugp \ge n^{-1-O(1/\log \log n)}$.


\subsection{Proof of \Cref{lem:relative-variance}}

The relative variance is defined as
\begin{align*} 
\frac{\mathbb E[X^2]}{\mathbb E^2[X]}-1
&\le\frac{\mathbb E[X^2]}{\mathbb E^2[X]}
\le\frac{(\max X)\mathbb E[X]}{\mathbb E^2[X]}
=\frac{\max X}{\mathbb E[X]}\\
&=\frac{\displaystyle\max_{C:\ell^{\mathcal T}(C)\le2\log n}p^{|C|}/q(C)}{\mathbb E[X]}
=\max_{C:\ell^{\mathcal T}(C)\le2\log n} \frac{p^{|C|}}{q(C)\cdot z'_G(p)} .\qedhere
\end{align*}





\subsection{Proof of \Cref{lem:reliable-main}}

We first establish a property of the sparsified $\widetilde{\mathcal T}$ that holds with high probability. We define a certain condition (namely~(\ref{eq:ji-log-ki-bound})) on each cut $C$ which we show holds with probability $\Omega(\delta)$ for a random tree $T\in\mathcal T$. 
Since the sparsified $\widetilde{\mathcal T}$ consists of $\tilde{O}(1)$ many random trees in $\mathcal T$, the probability that at least one $T\in\widetilde{\mathcal T}$ satisfies the condition is at least $1-n^{-10\log n}$. Since there are only $|\mathcal T|\cdot O(n^{8\log n})$ many possible cuts $C$ that can be returned by the sampler, by a union bound we conclude that at least one tree $T\in\mathcal T$ satisfies the condition for all cuts $C$ we need to consider.

Now consider a fixed cut $C\in\mathcal C$, and define $C_i=C\cap\widetilde E_i$. Sample a tree $T\in\widetilde{\mathcal T}$, and define $j^*_i=|C_i\cap E(T)|$ for all $i\in[L]$.

For all $i$, define $\tilde k'_{\pi_i} = \max\{\tilde k_{\pi_i}, \sqrt{n}\}$.
By \Cref{lem:tilde-ki-range}, 
\begin{gather}
\prod_i (\tilde k_{\pi_i}(T))^{j^*_i} \le \prod_i (\tilde k_{\pi_{i+2}})^{j^*_i}
\le \prod_i (\tilde k'_{\pi_{i+2}})^{j^*_i}
= \exp(\sum_i j^*_i \log \tilde k'_{\pi_{i+2}}).\label{eq:number-of-samples}
\end{gather}
For a given cut $C$, define $C_i=C\cap\widetilde E_i$. By definition, the load $\ell^{\mathcal T}(e)$ is the probability that a random tree $T\in\mathcal T$ contains edge $e$. Summing over all edges of $C_i$ and applying linearity of expectation, we obtain $\mathbb E_{T\sim\mathcal T}[j^*_i] = \ell^{\mathcal T}(C_i)$; note that this expectation is over a sample $T$ drawn from $\mathcal T$ instead of $\widetilde{\mathcal T}$. Summing $j^*_i\log \tilde k'_{\pi_{i+2}}$ over all $i$, we obtain
\[\mathop{\mathbb E}_{T\sim\mathcal T}[\sum_i j^*_i \log \tilde k'_{\pi_{i+2}}]
= \sum_i \ell^{\mathcal T}(C_i)\log \tilde k'_{\pi_{i+2}}.
\]
By Markov's inequality, at least a $\Omega(\delta)$ fraction of trees in $\mathcal T$ satisfy 
\begin{equation}\label{eq:ji-log-ki-bound}
    \sum_i j^*_i \log \tilde k'_{\pi_{i+2}} \le (1+\delta)\sum_i \ell^{\mathcal T}(C_i)\log \tilde k'_{\pi_{i+2}}.
\end{equation}
By our guarantee of $\widetilde{\mathcal T}$, at least one tree $T\in\widetilde{\mathcal T}$ also satisfies (\ref{eq:ji-log-ki-bound}).
In this case, we obtain
\[\frac 12 \log n \sum_i j^*_i \le \sum_i j^*_i \log \sqrt{n}\le \sum_i j^*_i \log \tilde k'_{\pi_{i+2}} \le (1+\delta)\sum_i \ell^{\mathcal T}(C_i) \log \tilde k'_{\pi_{i+2}} \le (1+\delta) \ell^{\mathcal T}(C) \log n,\]
which implies that $\sum_ij^*_i\le2(1+\delta)\ell^{\mathcal T}(C)$.
Since $\ell^{\mathcal T}(C)\le2 \log n$ and $\delta\le1$ by assumption, we have $\sum_i j^*_i \le8\log n$. In particular, it is possible for the algorithm to sample $j_i=j^*_i$ for all $i$. The probability that this occurs is the inverse of the number of combinations $j_1,j_2,\ldots,j_L$ satisfying $\sum_ij_i\le 8\log n$ and $j_i\le|E(T)\cap\widetilde E_i|$ for all $i\in[L]$. The first inequality alone limits the number of combinations to $(8\log n)^{O(L)}=(8\log n)^{O(1/\delta)}$, so the probability that $j_i=j^*_i$ for all $i$ is $(8\log n)^{-O(1/\delta)}$.

Conditioned on $j_i=j^*_i$ for all $i$, the cut $C$ is sampled precisely when we sample exactly the edges $C_i\cap E(T)$ from $\widetilde E_i\cap E(T)$ for each $i$. The total number of possible samples (over all $i$) is
\begin{align*}
\prod_i k_{\pi_i}^{j_i}=\prod_i k_{\pi_i}^{j^*_i}&\stackrel{(\ref{eq:number-of-samples})}\le  \exp(\sum_i j^*_i \log \tilde k'_{\pi_{i+2}})
 \\&\stackrel{(\ref{eq:ji-log-ki-bound})}\le \exp\bigg( (1+\delta)\sum_i \ell^{\mathcal T}(C_i)\log \tilde k'_{\pi_{i+2}}\bigg)
\\&=\prod_i(\tilde k'_{\pi_{i+2}})^{(1+\delta)\ell^{\mathcal T}(C_i)}
.
\end{align*}
Multiplying the probabilities together, the probability of sampling a tree $T\in\widetilde{\mathcal T}$ satisfying (\ref{eq:ji-log-ki-bound}), and then sampling $j_i=j^*_i$ for all $i$, and then sampling exactly the edges $C_i\cap E(T)$ from $\widetilde E_i\cap E(T)$ for each $i$ is at least
\[ \frac1{|\widetilde{\mathcal T}|} \cdot (8\log n)^{-O(1/\delta)} \cdot \prod_i(\tilde k'_{\pi_{i+2}})^{-(1+\delta)\ell^{\mathcal T}(C_i)} .\]
This is a lower bound for the probability $q(C)$ of sampling cut $C$. Note that since $|\widetilde{\mathcal T}|=\tilde O(1)$, the $1/|\widetilde{\mathcal T}|$ term can be absorbed into $(8\log n)^{-O(1/\delta)}$.

Finally, we bound the likelihood ratio 
\[\rho(C) = \frac{p^{|C|}}{q(C) \cdot z'}
    \le \frac{1}{z'} \cdot p^{|C|}\cdot(8\log n)^{O(1/\delta)}\cdot
    \prod_i (\tilde k'_{\pi_{i+2}})^{(1+\delta) \ell^{\mathcal T}(C_i)} .\]
Notice that
\[|C| = \sum_i |C_i| = \sum_i\sum_{e\in C_i}1\ge\sum_i\sum_{e\in C_i}\ell^{\mathcal T}(e)\pi_{i-1}
= \sum_i \ell^{\mathcal T}(C_i) \pi_{i-1}=\sum_i\ell^{\mathcal T}(C_i)\pi_{i-1} ,\]
so
\[\rho(C) \le \frac1{z'}\cdot\prod_ip^{\ell^{\mathcal T}(C_i)\pi_{i-1}}\cdot (8\log n)^{O(1/\delta)}\cdot
    \prod_i (\tilde k'_{\pi_{i+2}})^{(1+\delta) \ell^{\mathcal T}(C_i)} .\]

Recall from \Cref{lem:ugp-ktau} that $z\ge k_{\pi_{i+3}}p^{2\pi_{i+3}}$ for all $i$. We have $k_{\pi_{i+3}}\ge\tilde k_{\pi_{i+2}}$ by \Cref{lem:tilde-ki-range}, so we can write
\[ \frac1{z}=\prod_iz^{-\ell^{\mathcal T}(C_i)/\ell^{\mathcal T}(C)}\le\prod_i\big(\tilde k_{\pi_{i+2}}p^{2\pi_{i+3}}\big)^{-\ell^{\mathcal T}(C_i)/\ell^{\mathcal T}(C)}=\prod_i\big(\tilde k_{\pi_{i+2}}p^{2(1+\delta)\pi_{i+2}}\big)^{-\ell^{\mathcal T}(C_i)/\ell^{\mathcal T}(C)}, \]
and
\begin{align}
    \rho(C) &\le (8\log n)^{O(1/\delta)}\cdot \prod_i \left((\tilde k_{\pi_{i+2}}p^{2(1+\delta)\pi_{i+2}})^{-1/\ell^{\mathcal T}(C)}\cdot p^{\pi_{i-1}}\cdot(\tilde k'_{\pi_{i+2}})^{1+\delta}\right)^{\ell^{\mathcal T}(C_i)}\nonumber\\
    &=(8\log n)^{O(1/\delta)}\cdot \prod_i\left((\tilde k_{\pi_{i+2}})^{-1/\ell^{\mathcal T}(C)}\cdot p^{\pi_{i+2}\left(\frac1{(1+\delta)^3} - \frac{2(1+\delta)}{\ell^{\mathcal T}(C)}\right)}\cdot(\tilde k'_{\pi_{i+2}})^{1+\delta}\right)^{\ell^{\mathcal T}(C_i)}.\label{eq:rho-start}
\end{align}
Recall our assumption $n^{1+30\delta}\tilde k_{\pi_i}p^{2\pi_i}\le1$ for all $i$.
Notice that
\begin{align*}
(\tilde k'_{\pi_{i+2}})^{1+15\delta}=\max\{\tilde k_{\pi_{i+2}}, \sqrt{n}\}^{1+15\delta}
&\le (\sqrt{n\tilde k_{\pi_{i+2}}})^{1+15\delta}
= \sqrt{n^{1+15\delta}(k_{\pi_{i+2}})^{1+15\delta}}
\le \sqrt{n^{1+30\delta} k_{\pi_{i+2}}} \le p^{-\pi_{i+2}}.
\end{align*}
So, $p^{\pi_{i+2}}\le (\tilde k'_{\pi_{i+2}})^{-(1+15\delta)}$.
Let us first assume that $\ell^{\mathcal T}(C) \ge 2-\delta$, so the exponent $\frac1{(1+\delta)^3} - \frac{2(1+\delta)}{\ell^{\mathcal T}(C)}$ of $p^{\pi_{i+2}}$ is, for large enough constant $K>0$,
\[ \frac1{(1+\delta)^3} - \frac{2(1+\delta)}{\ell^{\mathcal T}(C)} = \frac1{(1+\delta)^3} -\frac{2(1+\delta)-K\delta}{\ell^{\mathcal T}(C)}-\frac{K\delta}{\ell^{\mathcal T}(C)} \ge \frac1{(1+\delta)^3}-\frac{2(1+\delta)-K\delta}{2-\delta}-\frac{K\delta}{\ell^{\mathcal T}(C)}\ge-\frac{K\delta}{\ell^{\mathcal T}(C)}. \]
We write
\begin{align*}
 p^{\pi_{i+2}\left(\frac1{(1+\delta)^3} - \frac{2(1+\delta)}{\ell^{\mathcal T}(C)}\right)}&=p^{\pi_{i+2}\left(\frac1{(1+\delta)^3} - \frac{2(1+\delta)}{\ell^{\mathcal T}(C)}+\frac{K\delta}{\ell^{\mathcal T}(C)}\right)}p^{\pi_{i+2}(-\frac{K\delta}{\ell^{\mathcal T}(C)})} 
\\&\le  (\tilde k'_{\pi_{i+2}})^{-(1+15\delta)\left(\frac1{(1+\delta)^3} - \frac{2(1+\delta)}{\ell^{\mathcal T}(C)}+\frac{K\delta}{\ell^{\mathcal T}(C)}\right)}p^{\pi_{i+2}(-\frac{K\delta}{\ell^{\mathcal T}(C)})}
\\&=  (\tilde k'_{\pi_{i+2}})^{-\frac{1+15\delta}{(1+\delta)^3} + \frac{2+O(\delta)}{\ell^{\mathcal T}(C)}-\frac{K\delta}{\ell^{\mathcal T}(C)}}p^{\pi_{i+2}(-\frac{K\delta}{\ell^{\mathcal T}(C)})}
\\&\le  (\tilde k'_{\pi_{i+2}})^{-(1+\delta)+ \frac{2+O(\delta)}{\ell^{\mathcal T}(C)}-\frac{K\delta}{\ell^{\mathcal T}(C)}}p^{\pi_{i+2}(-\frac{K\delta}{\ell^{\mathcal T}(C)})} ,
\end{align*}
where the first inequality uses the fact that the new exponent $\frac1{(1+\delta)^3} - \frac{2(1+\delta)}{\ell^{\mathcal T}(C)}+\frac{K\delta}{\ell^{\mathcal T}(C)}$ is nonnegative, and the second inequality uses $1+15\delta\ge(1+\delta)^4$ since $\delta\le1$. Continuing from (\ref{eq:rho-start}), we are left with
\begin{align*}
\rho(C)&\le(8\log n)^{O(1/\delta)}\cdot \prod_i \left((\tilde k_{\pi_{i+2}})^{-1/\ell^{\mathcal T}(C)} (\tilde k'_{\pi_{i+2}})^{\frac{2+O(\delta)}{\ell^{\mathcal T}(C)}}(\tilde k'_{\pi_{i+2}}p^{\pi_{i+2}})^{\frac{-K\delta}{\ell^{\mathcal T}(C)}}\right)^{\ell^{\mathcal T}(C_i)}
\\&=(8\log n)^{O(1/\delta)}\cdot \prod_i \left((\tilde k_{\pi_{i+2}})^{-1} (\tilde k'_{\pi_{i+2}})^{2+O(\delta)}\right)^{\frac{\ell^{\mathcal T}(C_i)}{\ell^{\mathcal T}(C)}}\cdot\prod_i\left(\tilde k'_{\pi_{i+2}}p^{\pi_{i+2}}\right)^{-K\delta\cdot\frac{\ell^{\mathcal T}(C_i)}{\ell^{\mathcal T}(C)}} .
\end{align*}
For the first product, we use the bound $\tilde k'_{\pi_{i+2}}=\max\{\tilde k_{\pi_{i+2}}, \sqrt{n}\}\le\sqrt{n\tilde k_{\pi_{i+2}}}$ to get
\begin{align*}
\prod_i \left((\tilde k_{\pi_{i+2}})^{-1} (\tilde k'_{\pi_{i+2}})^{2+O(\delta)}\right)^{\frac{\ell^{\mathcal T}(C_i)}{\ell^{\mathcal T}(C)}}&\le\prod_i \left((\tilde k_{\pi_{i+2}})^{-1} \big(\sqrt{n\tilde k_{\pi_{i+2}}}\big)^{2+O(\delta)}\right)^{\frac{\ell^{\mathcal T}(C_i)}{\ell^{\mathcal T}(C)}}
\\&= \prod_i \left( (\tilde k_{\pi_{i+2}})^{O(\delta)} n^{1+O(\delta)}\right)^{\frac{\ell^{\mathcal T}(C_i)}{\ell^{\mathcal T}(C)}}
\\&\le\prod_i\left(n^{1+O(\delta)}\right)^{\frac{\ell^{\mathcal T}(C_i)}{\ell^{\mathcal T}(C)}}
\\&=n^{1+O(\delta)} .
\end{align*}
For the second product, we use the fact that $\pi_i\in\Theta(\lambda)$ and our assumption $p^\lambda\ge n^{-1000}$ to obtain
\[ \prod_i(\tilde k'_{\pi_{i+2}}p^{\pi_{i+2}})^{-K\delta\cdot\frac{\ell^{\mathcal T}(C_i)}{\ell^{\mathcal T}(C)}}\le\prod_i( n^{-O(1)})^{-K\delta\cdot\frac{\ell^{\mathcal T}(C_i)}{\ell^{\mathcal T}(C)}}=(n^{-O(1)})^{-K\delta}=n^{O(\delta)} .\]
We conclude that $\rho(C)\le(\log n)^{O(1/\delta)}n^{1+O(\delta)}$ under the additional assumption that $\ell^{\mathcal T}(C) \ge 2-\delta$.

To handle the case $\ell^{\mathcal T}(C)<2-\delta$, observe that by Markov's inequality, at least a $\Omega(\delta)$ fraction of trees $T\in\mathcal T$ satisfy $|C\cap E(T)|<2$, which means $|C\cap E(T)|=1$. We can similarly argue, as in the beginning of the proof, that with high probability at least one tree $T\in\widetilde{\mathcal T}$ satisfies $|C\cap E(T)|=1$. Now suppose that the single edge in $C\cap E(T)$ is in $\widetilde E_i$. Then, with probability $(8\log n)^{-O(1/\delta)}$ we have $j_i=1$ and $j_{i'}=0$ for all $i'\ne i$, and with probability $1/|\widetilde E_i\cap E(T)|\ge1/n$. So overall, the cut $C$ is sampled with probability $1/|\widetilde{\mathcal T}|\cdot(8\log n)^{-O(1/\delta)}\cdot1/n$. It follows that
\[ \rho(C)=\frac{p^{|C|}}{q(C)\cdot z'_G(p)}\le\frac1{q(C)}=(8\log n)^{O(1/\delta)}\cdot n ,\]
concluding the proof.


\subsection{Proof of \Cref{lem:very-reliable-bias}}

By the standard cut-counting bound, we have
    \begin{align*}
    \frac1z\sum_{|C|\ge 1.1\lambda}p^{|C|} &= \frac1z\bigg(\sum_{1.1\lambda\le|C|\le2\lambda}p^{|C|}+\sum_{|C|>2\lambda}p^{|C|}\bigg)\\
    &\le p^{-\lambda}\bigg(n^4p^{1.1\lambda}+\sum_{j\ge2}n^{2(j+1)}p^{j\lambda}\bigg)\\
    &\le n^4 p^{0.1\lambda} + n^4\sum_{j\ge 2} n^{2(j-1)} p^{(j-1)\lambda}\\
    &\le n^4p^{0.1\lambda}+n^4\sum_{j\ge2}(n^2p^\lambda)^{j-1},
    \end{align*}
which is $O(1/n)$ since $p^\lambda < n^{-1000}$.

\subsection{Proof of \Cref{lem:very-reliable-likelihood-ratio}}

We start with the following claim:

\begin{claim}\label{claim:reliable-case-greedy-load-approx}
    The following holds with high probability: $\ell_i(e)\le 1.01\ell^*(e)$ for each $i\in\{1,2,\ldots,\log\log n+1\}$ and each $e\in E(G_i)$.
\end{claim}

\begin{proof}
By \Cref{lem:monotone}, contraction can only decrease ideal loads of remaining edges, so the ideal loads $\ell^*_i$ in $G_i$ satisfy $\ell^*_i(e)\le \ell^*(e)$ for $e\in E(G_i)$.
Since $\ell_i \approx_{0.01}\ell^*_i$, we have $\ell_i(e)\le 1.01\ell^*_i(e) \le 1.01\ell^*(e)$ for all $e\in E(G_i)$.
\end{proof}

This claim is now used to establish the next claim:

\begin{claim}
    For each $i\in\{1,2,\ldots,\log\log n+1\}$, if $|C|\in [c_{k_i}, c_{k_{i+1}})$ and $|C|<1.1\lambda$, then $\frac{1}{q(C)} \le \tilde{O}(1) \cdot k_{i+1}^2$.
\end{claim}
\begin{proof}
    Because $|C|<c_{k_{i+1}}$, $C$ does not separate any $c_{k_{i+1}}$-connected components of $G$. Because $G_{i+1}$ is formed by contracting $c_{k_{i+1}}$-connected components, $C$ is preserved in $G_{i+1}$. (In the case $i=\log\log n$, note that $G_{\log \log n+1}$ is the original graph.)

    The above argument also implies that the min-cut of $G$ is preserved in $G_{i+1}$. Combined with the fact that contraction cannot decrease min-cut value, we have that the min-cut value in $G_{i+1}$ is still $\lambda$. Thus, the ideal tree packing value $\pi^*_{i+1} > \frac{2}{\lambda}$ by \Cref{fact:pi-range}.
    Because $|C|< 1.1\lambda$, we have $\ell^*_{i+1}(C) \le |C|/\pi^*_{i+1} < 2|C|/\lambda < 2.2$.
    By \Cref{claim:reliable-case-greedy-load-approx}, in greedy tree packing $\mathcal T_{i+1}$, $\ell_{i+1}(C)\le 1.01\ell^*_{i+1}(C)< 2.3$. Notice that $\ell_{i+1}(C)=\mathbb E[|T\cap C|]$ for a uniformly random tree $T$ in $\mathcal T_{i+1}$. By Markov's inequality, $\Pr[|T\cap C|\ge 3] < \frac{2.3}{3}<0.8$, which implies $\Pr[|T\cap C|\le 2]>0.2$. Since $\widetilde{\mathcal T}_{i+1}$ is a random sample of $\tilde{O}(1)$ trees in $\mathcal T_{i+1}$, with high probability there exists some $T\in\widetilde{\mathcal T}_{i+1}$ such that $|T\cap C|\le 2$. Moreover, this holds with high probability over all cuts $C$ with $|C|<1.1\lambda$ since there are only $n^{O(1)}$ such cuts.

    Given a tree $T\in\widetilde{\mathcal T}_{i+1}$ with $|T\cap C|\le2$, the cut $C$ can be sampled if the one or two edges in $T\cap C$ are sampled by the algorithm. This happens with probability $\frac{1}{k_{i+1}^2}$. So overall, $q(C)\ge\frac1{\log\log n+1}\cdot\frac1{|\widetilde{\mathcal T}_{i+1}|} \cdot \frac{1}{k_{i+1}^2}$, where the first and second factor come from sampling the correct $i$ and $T\in\widetilde{\mathcal T}_{i+1}$. Rearranging and using $|\widetilde{\mathcal T}_{i+1}|=\tilde{O}(1)$ finishes the proof. %(Even when $|T\cap C|=1$, we sample it with the same probability because the sampling is with replacement.)
%    $q$ is the average of $\tO(1)$ distributions, so $\frac{1}{q(C)} \le \tO(1) \cdot \frac{1}{q_{(i+1, T)}(C)} \le \tO(1) \cdot k_{i+1}^2$.
\end{proof}

Finally, we need the following claim:

\begin{claim}
    $z'_G(p) \ge k_i p^{c_{k_i}}$ for all $i\in\{1,2,\ldots,\log\log n+1\}$. %$i=1, 2, \ldots, \log \log n$.
\end{claim}
\begin{proof}
    In the list of Gomory-Hu tree cuts, $c_{k_i}$ is the $k_i$-th smallest cut, so there are $k_i$ distinct cuts of value $\le c_{k_i}$. Their contribution to $z'_G(p)$ is at least $k_i p^{c_{k_i}}$.
\end{proof}

To prove \Cref{lem:very-reliable-likelihood-ratio},
we bound the likelihood ratio for all cuts $C$ with $|C|<1.1\lambda$ by combining the above claims.
Suppose $|C|\in[c_{k_i}, c_{k_{i+1}})$. We have
\begin{align*}
    \frac{p^{|C|}}{q(C)\cdot z'_G(p)}\le p^{c_{k_i}}\cdot \frac{1}{q(C)} \cdot \frac{1}{k_i p^{c_{k_i}}}
    \le \frac{\tilde{O}(1)\cdot k_{i+1}^2}{k_i} = \tilde{O}(1)\cdot n^{2(1-2^{-i-1}) - (1-2^{-i})} = \tilde{O}(n).
\end{align*}
We have covered the whole range $[\lambda, 1.1\lambda)$ because $c_{k_0}=c_1=\lambda$ and $c_{k_{\log \log n+1}}=c_n = \max\{1.1\lambda,c_{n-1}\}\ge1.1\lambda$.



\section{Omitted Proofs from \Cref{sec:contraction}}
\label{sec:proof4}

\subsection{Proof of \Cref{fact:gamma-star-to-gamma}}
    By definition, contracting edges with $\ell^*(e) \le 1/\gamma^*$ gives $< \delta n$ nodes but contracting edges with $\ell^*(e) \le 1/\gamma^*$ gives $\ge \delta n$ nodes. Now, we note the following:
    \begin{enumerate}
        \item First, for any edge $e$, if $\ell^*(e) \le 1/\gamma^*$, then $\ell(e) \le (1+\delta)/\gamma^*$. Therefore, contracting all edges with $\ell(e) \le (1+\delta)/\gamma^*$ also yields at most $\delta n$ nodes. Hence, $\gamma' \ge \gamma^*/(1+\delta)$.
        \item Next, suppose we contract all edges $e$ with $\ell(e) < (1-\delta)/\gamma^*$. All these edges have  $\ell^*(e) < 1/\gamma^*$. Therefore, this contraction will yield $\ge \delta n$ nodes. Therefore, $\gamma' \le \gamma^*/(1-\delta)$. \qedhere
    \end{enumerate}


\subsection{Proof of \Cref{fact:u-to-p-gamma}}


There are two cases depending on whether $\gamma=\lambda$ or $\gamma = \gamma'$.
In the first case, we have $\ugp \ge p^\lambda \ge p^{(1+O(1/\log \log n))\lambda}$.

In the second case, we first note that $\ugp \ge n^{-1-O(1/\log \log n)}$ also implies $\ugp \ge (\delta n)^{-1-\Theta(1/\log \log n)}$ since
\[
\delta^{-1-\Theta(1/\log \log n)} 
\le O(\log\log n)^{1+O(1/\log \log n)}
\le n^{O(1/\log\log n)}.
\]
Next, recall that $k_{\tau}$ is the number of nodes after contracting all edges $e$ with $\ell^*(e) < 1/\tau$.
    By \Cref{lem:ugp-ktau} and \Cref{fact:gamma-star-to-gamma}, 
    \[
        \ugp\ge k_{\gamma^*} p^{2\gamma^*}\ge \delta n \cdot p^{2(1+\delta)\gamma}.
    \]
    We combine this with $\ugp\ge (\delta n)^{-1-\Theta(1/\log \log n)}$, which is equivalent to 
    \[
        (\ugp)^{1+\Theta(1/\log \log n)} \ge (\delta n)^{-1}.
    \]
    
    Multiplying the two inequalities above, we get 
    \[
        (\ugp)^{2+\Theta(1/\log \log n)} \ge   p^{2(1+\delta)\gamma}.
    \]
    Therefore, $(\ugp)^2 \ge p^{2(1+\delta)\gamma}$, or equivalently, 
    $\ugp \ge p^{(1+\delta)\gamma}$.






\subsection{Proof of \Cref{lem:size-dec-cluster}}
    Consider a continuous-time random process where each edge independently arrives at a time $t_e$, and the arrival times follow independent exponential distributions of rate 1. Let $G_t$ be the random graph formed by contracting all edges arriving up to time $t$. Let $n_t$ and $m_t$ be the number of vertices and edges in $G_t$ respectively. We consider how $n_t$ evolves during the process. Let $t(k)$ be the first time when $n_t\le k$. Initially $n_0=n$ and $t(n)=0$. Now, $n_t$ decreases by 1 whenever an uncontracted edge (i.e., an edge whose endpoints are vertices that haven't been contracted to the same node yet) arrives. Since there are $m_t$ uncontracted edges at time $t$, the earliest arrival time of an uncontracted edge after time $t$ follows an exponential distribution of rate $m_t$. 
    After any edge contraction, the nodes form a partition of $G$. Thus, $\frac{m_t}{n_t-1}\ge \pi$.

    Let $\Delta_k = t(k-1)-t(k)$. As discussed above, $\Delta_k$ follows an exponential distribution of rate $m_{t(k)}\ge \pi(k-1)$.
    Next, we couple each $\Delta_k$ with a new random variable defined by the aforementioned contraction process on a star graph. Let $R$ be a star on $n$ vertices and $n-1$ edges. We use the same notations as above for graph $R$, but with a superscript of $R$. Note that during the contraction process, we always have $m_t^R = n_t^R-1$.
    Therefore, $\Delta_k^R=t^R(k-1)-t^R(k)$ follows an exponential distribution of rate $k-1$.
    Let $\Delta'_k = \Delta_k^R / \pi$. Then, $\Delta'_k$ follows an exponential distribution of rate $(k-1)\pi$.
    Because of the memoryless property of exponential distributions and the independence of edges, $\Delta_k$ or $\Delta^R_k$ for different $k$ are independent.
    We can couple $\Delta_k$ and $\Delta'_k$ so that each $\Delta_k$ is stochastically dominated by $\Delta'_k$.
    Then,
    \[t(k)=t(k)-t(n) = \sum_{i=k+1}^n \Delta_i \le
    \sum_{i=k+1}^n \Delta'_i 
    = \sum_{i=k+1}^n \frac{\Delta^R_i}{\pi} = \frac{t^R(k)}{\pi}\]
    This implies $n_t \le n^R_{\pi t}$.

    The size of $G(q)$ is $n_{-\ln q}$, which is upper bounded by $n^R_{-\pi \ln q}$. $n^R_{-\pi \ln q}$ is the vertex size of $R$ after contracting each edge with probability $1-q^\pi$.
    So, its expectation is $1+q^{\pi}(n-1)$. % = 1 + \frac 12 (n-1)$.
    By Hoeffding's inequality, $\Pr[|V(H)|> 1+(1+\eps)q^{\pi} n] \le \exp(-\Omega(\eps^2 n))$.








\subsection{Proof of \Cref{lem:relvar-1step}}

%We abbreviate $\ugp$ by $u$ in this proof.
We abbreviate cut value $|C_i|$ by $c_i$ in the proof.
By \Cref{fact:u-to-p-gamma}, we have that $\ugp\ge p^{(1+\delta)\gamma}$.
Let $\tilde{\gamma}=(1+\delta)\gamma$ such that $\ugp\ge p^{\tilde{\gamma}}$.
Then 
\[
    q^{-\tilde{\gamma}}
    = 2^{1+\delta} 
    = 2^{1 + O(1/\log\log n)}
    = 2+O(1/\log \log n).
\]

The relative second moment is bounded as:
\begin{align*}
\frac{\E[z_H(p/q)^2]}{(\zgp)^2}
&= \frac{1}{(\zgp)^2}\cdot \E\bigg[\sum_{C_i, C_j \in \mathcal{C}(H)}\left(\frac{p}{q}\right)^{c_i+c_j}\bigg] 
= \frac{1}{(\zgp)^2}\sum_{C_i, C_j\in \mathcal{C}(G)} q^{|C_i\cup C_j|}\cdot \left(\frac{p}{q}\right)^{c_i+c_j}\\
&= \frac{1}{(\zgp)^2}\left(\sum_{C_i}\frac{p^{2c_i}}{q^{c_i}} + \sum_{C_i\ne C_j: |C_i\cap C_j|\le \tilde{\gamma}} \frac{p^{c_i+c_j}}{q^{|C_i\cap C_j|}} + \sum_{C_i\ne C_j: |C_i\cap C_j| > \tilde{\gamma}} \frac{p^{c_i+c_j}}{q^{|C_i\cap C_j|}}\right).
\end{align*}
In the above expression, we distinguished between the cases $C_i = C_j$ and $C_i \ne C_j$, and the second case is further split into $|C_i \cap C_j| \le \tilde{\gamma}$ and $|C_i\cap C_j| > \tilde{\gamma}$. We define:
\begin{align*}
    V_1 &= \sum_{C_i}\frac{p^{2c_i}}{q^{c_i}}\\
    V_2 &= \sum_{C_i\ne C_j: |C_i\cap C_j|\le \tilde{\gamma}} \frac{p^{c_i+c_j}}{q^{|C_i\cap C_j|}}\\
    V_3 &= \sum_{C_i\ne C_j: |C_i\cap C_j| > \tilde{\gamma}} \frac{p^{c_i+c_j}}{q^{|C_i\cap C_j|}}.
\end{align*}

We first bound $V_1$:


\[
V_1 - q^{-\tilde{\gamma}}\sum_{C_i} p^{2c_i}
= \sum_{C_i} p^{2c_i}\left(\frac{1}{q^{c_i}} - \frac{1}{q^{\tilde{\gamma}}}\right)
= \frac{p^{\tilde{\gamma}}}{q^{\tilde{\gamma}}} \sum_{C_i} p^{c_i} \cdot p^{c_i-\tilde{\gamma}}(q^{-(c_i-\tilde{\gamma})}-1).
%= \frac{p^{\tilde{\gamma}}}{q^{\tilde{\gamma}}}  \sum_{C_i} p^{c_i} \cdot p^{c_i-\tilde{\gamma}}(q^{-(c_i-\tilde{\gamma})}-1)
\]

Let us also denote $t_i=\frac{c_i-\tilde{\gamma}}{\tilde{\gamma}}$ and $f(t)=(q^{-\tilde{\gamma}}\cdot w)^t-w^t = p^{c_i-\tilde{\gamma}}(q^{-(c_i-\tilde{\gamma})}-1)$ where $w=p^{\tilde{\gamma}}$. Therefore, 
\[
    V_1 - q^{-\tilde{\gamma}}\sum_{C_i} p^{2c_i} = \frac{p^{\tilde{\gamma}}}{q^{\tilde{\gamma}}} \sum_{C_i} p^{c_i}\cdot f(t_i).
\]
\begin{fact}
    Suppose $0 < w \le n^{-\Omega(1/\log \log n)}$ and $2 \le \alpha \le e$. Function $f(t)=(\alpha w)^t-w^t$ has global maximum $\le O\left(\frac{\log \log n}{\log n}\right)$.
\end{fact}
\begin{proof}
Let $f'(t) = (ew)^t-w^t\ge f(t)$.
    \begin{align*}
    \frac{df}{dt}
    &= (ew)^t \ln (ew) - w^t \ln w
    = e^t w^t \left(1 - (1-e^{-t})\ln\frac{1}{w}\right).
\end{align*}
$\frac{df}{dt}=0$ at $t^*=\ln\left(\frac{\log w}{\log (ew)}\right)$.
Notice that $1 - (1-e^{-t})\ln\frac{1}{w}$ is monotone decreasing, so $\frac{df}{dt}\ge 0$ when $t<t^*$ and $\frac{df}{dt}\le 0$ when $t>t^*$. Thus, $f(t^*)$ is a global maximum.

We now calculate the value of the global maximum. First, we get
\[e^{t^*}-1 = \frac{\log w}{\log (ew)}-1 = -\frac{1}{\ln (ew)}  \le O\left(\frac{\log \log n}{\log n}\right). \]
We have $w^{t^*}\le 1$ because $w\in(0,1)$ and $t^*>0$. So $f(t^*) \le w^{t^*}(e^{t^*}-1) \le O\left(\frac{\log \log n}{\log n}\right)$.
\end{proof}

Combining this fact with $p^{\tilde{\gamma}}\le \ugp\le\zgp$, $q^{-\tilde{\gamma}} = O(1)$, and $\zgp = \sum_{C_i} p^{c_i}$, we get
\begin{align}\label{eq:v1}
    V_1 - q^{-\tilde{\gamma}}\sum_{C_i}p^{2c_i}
    %\le O(1) \cdot (\zgp)^2 \cdot O\left(\frac{\log \log n}{\log n}\right) 
    \le O\left(\frac{\log \log n}{\log n}\right) \cdot (\zgp)^2.
\end{align}

Next, we bound $V_2$ as follows:
\begin{align}\label{eq:v2}
V_2 
= \sum_{C_i\ne C_j, |C_i\cap C_j|\le \tilde{\gamma}} \frac{p^{c_i+c_j}}{q^{|C_i\cap C_j|}}
\le q^{-\tilde{\gamma}}\cdot \sum_{C_i, C_j} p^{c_i+c_j} - q^{-\tilde{\gamma}}\cdot \sum_{C_i} p^{2c_i}
= q^{-\tilde{\gamma}}\cdot (\zgp)^2 - q^{-\tilde{\gamma}}\cdot \sum_{C_i} p^{2c_i}.
\end{align}

Finally, we bound $V_3$.
Recall that $x_G(p)$ is the expected number of failed cut pairs in \Cref{lem:z-approx-u}.
\[
V_3 
= \sum_{C_i\ne C_j, |C_i\cap C_j|>\tilde{\gamma}} p^{|C_i\cup C_j|}\left(\frac{p}{q}\right)^{|C_i\cap C_j|}
\le \sum_{C_i\ne C_j} p^{|C_i\cup C_j|}\left(\frac{p}{q}\right)^{\tilde{\gamma}}
= q^{-\tilde{\gamma}} \cdot x_G(p)\cdot p^{\tilde{\gamma}} 
\le q^{-\tilde{\gamma}}\cdot x_G(p) \cdot \zgp.
\]
Since $p< \theta$, \Cref{lem:z-approx-u} gives $x_G(p) \le \frac{1}{\log n}\cdot \zgp$. Therefore,
\begin{align}\label{eq:v3}
    V_3 \le  q^{-\tilde{\gamma}}\cdot x_G(p) \cdot \zgp \le \frac{3}{\log n}\cdot (\zgp)^2.
\end{align}    

Putting the bounds on $V_1, V_2$ and $V_3$ given by \eqref{eq:v1}, \eqref{eq:v2}, and \eqref{eq:v3} together, we get
\[
\frac{\E[z_H(p/q)^2]}{(\zgp)^2} 
\le \frac{V_1+V_2+V_3}{(\zgp)^2}  
= 2 + O\left(\frac{\log \log n}{\log n}\right).\qedhere
\]








\subsection{Proof of \Cref{lem:runtime-sparsify-step}}

Sparsification generates a graph $H$ with min-cut value $\lambda_H=\tO(1)$. Then we perform random contraction on $H$ with $q^{\gamma_H} = \nicefrac 12$. Because we defined $\gamma_H\le \lambda_H$, we have $\frac{1}{1-q} = O(\gamma_H) = O(\lambda_H)$. By \Cref{lem:kkt-contraction-size-bound}, the expected edge size of the graph after contraction is at most $\E[m'] = \frac{n}{1-q}= O(n\cdot \lambda_H) = \tO(n)$. (Note that $n$ is the vertex size before sparsification.)

Under the assumption $m > n^{1+\Omega(\frac{1}{\sqrt{\log n}})}$, we have $\E[m'] \le \tO(n) \le m^{1-\Omega\left(\frac{1}{\sqrt{\log n}}\right)}$. Notice that $x^a$ is concave when $a\in(0,1)$ and we can apply Jensen's inequality.
\[
\E\left[(m')^{\frac{1}{\sqrt{\log n}}}\right]
\le \left(\E[m']\right)^{\frac{1}{\sqrt{\log n}}}
\le m^{\left(1-\Omega\left(\frac{1}{\sqrt{\log n}}\right)\right)\frac{1}{\sqrt{\log n}}}
= m^{\frac{1}{\sqrt{\log n}}} \cdot m^{-\Omega\left(\frac{1}{\log n}\right)}
\le \nf 12 \cdot m^{\frac{1}{\sqrt{\log n}}},
\]
when the constant in the $O(\cdot)$ of the assumption in the lemma's statement statement is sufficiently large.

